Geometry Processing of Conventionally Produced Mouse Brain Slice Images

Brain mapping research in most neuroanatomical laboratories relies on conventional processing techniques, which often introduce histological artifacts such as tissue tears and tissue loss. In this paper we present techniques and algorithms for automatic registration and 3D reconstruction of conventionally produced mouse brain slices in a standardized atlas space. This is achieved first by constructing a virtual 3D mouse brain model from annotated slices of Allen Reference Atlas (ARA). Virtual re-slicing of the reconstructed model generates ARA-based slice images corresponding to the microscopic images of histological brain sections. These image pairs are aligned using a geometric approach through contour images. Histological artifacts in the microscopic images are detected and removed using Constrained Delaunay Triangulation before performing global alignment. Finally, non-linear registration is performed by solving Laplace's equation with Dirichlet boundary conditions. Our methods provide significant improvements over previously reported registration techniques for the tested slices in 3D space, especially on slices with significant histological artifacts. Further, as an application we count the number of neurons in various anatomical regions using a dataset of 51 microscopic slices from a single mouse brain. This work represents a significant contribution to this subfield of neuroscience as it provides tools to neuroanatomist for analyzing and processing histological data.

==> conclusion.tex <==
\section{Conclusion}
\label{conclusion}



%Neural circuit mapping based on conventionally processed brain sections is riddled with histological artifacts and is the most common form of data used in almost all neuroanatomical laboratories.  An accurate, robust, and automatic registration algorithm that we propose to handle such data will open up endless possibilities of new research in all such laboratories.


%Such an automated registration would enable automatic identification and quantification of neuronal activity in each annotated regions along with inter-specimen comparisons. Bringing such damaged datasets into a common anatomical framework enables the creation of a more complete and accessible database.


To encourage development, validation, and comparison, we release model

To the best of our knowledge the presented work is the first that automatically registers highly damaged high-resolution optical images of mouse brain to hand-drawn atlas contours without using any intermediate atlas. 

We believe that this work will have a major impact on brain circuit mapping by facilitating conventional neuroanatomical image registration and creation of 3D whole brain map databases. 

==> implementation.tex <==
\section{Implementation}
\label{implementation}

values for median and gaussian filter for smootheninig

median filter size =[20 20]
gaussian filter size 12, std 2

threshold computation
In our implementation we found best results for $s=12$, for which $k=5$. 

for damaged region detection
we use $\alpha=20$

The complete algorithm to align a damaged histological slice with its cor- responding ARA maps takes 1 minute with our unoptimized MATLAB code on an Intel Core i5 CPU with 8GB RAM. 

%For quicker convergence, in each successive iteration we reduce the neighborhood by half and the angle threshold by 20$\%$. Empirically we found out that four iterations with angle threshold of $\left(10^{\circ}, 8^{\circ}, 6^{\circ}, 4^{\circ}\right)$ and distance threshold of $\left(\frac{1}{10},\frac{1}{20},\frac{1}{40},\frac{1}{80}\right)$ of image height gave the best results.
We used progressively tighter normal vector angle deviation thresholds $\left(10^{\circ}, 8^{\circ}, 6^{\circ}, 4^{\circ}\right)$ and smaller distance threshold $\left(\frac{1}{10},\frac{1}{20},\frac{1}{40},\frac{1}{80} \right)$ of image-height in each iteration for quicker convergence.


Surface fairing : $\lambda$ and $\mu$ values

We use this algorithm only on the green channel of the MI as it comes from auto-fluorescence which reflects the overall structural of the slice.   

%\subsection{Specimen Preparation \& Data Acquisition}
%Recombinant Adeno-Associated Virus (rAAV) expressing EGFP were used to label specific neuronal projections in the mouse brains. Please see \cite{Sun:2014aa,Oh:2014aa} for detailed experimental procedures.  
%
%For histological processing, the mice brains were sectioned coronally in 30$\mu m$ thickness on a freezing microtome. Brain slices were counter-stained with 10 $\mu M$ DAPI, then mounted and cover-slipped.  A whole series of brain slices were imaged using the Automated Slide Scanning and Analysis software (Metamorph, Inc.) in a high-capacity computer coupled with a fluorescent BX61 Olympus microscope through a 10X objective and a high-sensitive Hamamatsu CCD camera. Image stitching, overlaying were completed by using Metamorph imaging and analysis tools. 
%
%
%To generate the microscopic slices, the mice brains 



